Spatially constrained vs. unconstrained filtering in neural spatiospectral filters for multichannel speech enhancement

When using artificial neural networks for multichannel speech enhancement, filtering is often achieved by estimating a complex-valued mask that is applied to all or one reference channel of the input signal. The estimation of this mask is based on the noisy multichannel signal and, hence, can exploit spatial and spectral cues simultaneously. While it has been shown that exploiting spatial and spectral cues jointly is beneficial for the speech enhancement result, the mechanics of the interplay of the two inside the neural network are still largely unknown. In this contribution, we investigate how two conceptually different neural spatiospectral filters (NSSFs) exploit spatial cues depending on the training target signal and show that, while one NSSF always performs spatial filtering, the other one is selective in leveraging spatial information depending on the task at hand. These insights provide better understanding of the information the NSSFs use to make their prediction and, thus, allow to make informed decisions regarding their design and deployment.

==> figures/FTJNF-fix-dry/figure_FTJNFfix_Dry_A4.tex <==
\begin{figure}
\centering
    \begin{subfigure}[t,right]{\columnwidth}
        \subcaption{Features $\bh_1(\tau)$}
        \input{figures/FTJNF-fix-dry/20_lstm1_features.tikz}
        \label{subfig:ftjnf_dry_a4_features_lstm1}
    \end{subfigure}
     \vspace{-.3cm} 
     
    \begin{subfigure}[t,right]{\columnwidth}
        \subcaption{Features $\bh_2(\tau)$}
        \input{figures/FTJNF-fix-dry/20_lstm2_features.tikz}
        \label{subfig:ftjnf_dry_a4_features_lstm2}
    \end{subfigure}
    
     \vspace{-.3cm} 
    \begin{subfigure}[t,right]{\columnwidth}
        \subcaption{Clustering result $\bh_1(\tau)$}
        \input{figures/FTJNF-fix-dry/20_lstm1_clusters_mode_1.tikz}
        \label{subfig:ftjnf_dry_a4_clusters_lstm1}
    \end{subfigure}

     \vspace{-.3cm} 
    \begin{subfigure}[t,right]{\columnwidth}
        \subcaption{Clustering result $\bh_2(\tau)$}
        \input{figures/FTJNF-fix-dry/20_lstm2_clusters_mode_1.tikz}
        \label{subfig:ftjnf_dry_a4_clusters_lstm2}
    \end{subfigure}

    \vspace{-.3cm}
    \begin{subfigure}[t,right]{\columnwidth}
        \subcaption{Input signal}
        \input{figures/FTJNF-fix-dry/20_input.tikz}
        \label{subfig:ftjnf_dry_a4_input}
    \end{subfigure}
    
    % \vspace{-.3cm}
    % \begin{subfigure}[t,right]{\columnwidth}
    %     \subcaption{Target signal}
    %     \input{figures/FTJNF-fix/Dry/20_target.tikz}
    %     \label{subfig:ftjnf_dry_a4_target}
    % \end{subfigure}
        	
    \caption{Exemplary feature maps of (a) $\bh_1(\tau)$ and (b) $\bh_2(\tau)$ of the \ac{JNF}-Dry, and  (c, d) the respective clustering result (P: Pause, $1$: Position $1$, $2$: Position $2$) and (e) time-domain input signal. The fixed target speaker position for Speaker~$1$ is at $90$\degree, Speaker~$2$ at $12$\degree. The red lines indicate the position change.}
    \label{fig:ftjnffix_dry_a4} 	
\end{figure}
